The Decentralized Financial Crisis

The Global Financial Crisis of 2008, caused by the accumulation of excessive financial risk, inspired Satoshi Nakamoto to create Bitcoin. Now, more than ten years later, Decentralized Finance (DeFi), a peer-to-peer financial paradigm which leverages blockchain-based smart contracts to ensure its integrity and security, contains over 702m USD of capital as of April 15th, 2020. As this ecosystem develops, it is at risk of the very sort of financial meltdown it is supposed to be preventing. In this paper we explore how design weaknesses and price fluctuations in DeFi protocols could lead to a DeFi crisis. We focus on DeFi lending protocols as they currently constitute most of the DeFi ecosystem with a 76% market share by capital as of April 15th, 2020. First, we demonstrate the feasibility of attacking Maker's governance design to take full control of the protocol, the largest DeFi protocol by market share, which would have allowed the theft of 0.5bn USD of collateral and the minting of an unlimited supply of DAI tokens. In doing so, we present a novel strategy utilizing so-called flash loans that would have in principle allowed the execution of the governance attack in just two transactions and without the need to lock any assets. Approximately two weeks after we disclosed the attack details, Maker modified the governance parameters mitigating the attack vectors. Second, we turn to a central component of financial risk in DeFi lending protocols. Inspired by stress-testing as performed by central banks, we develop a stress-testing framework for a stylized DeFi lending protocol, focusing our attention on the impact of a drying-up of liquidity on protocol solvency. Based on our parameters, we find that with sufficiently illiquidity a lending protocol with a total debt of 400m USD could become undercollateralized within 19 days.

==> content/contagion.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=\columnwidth]{images/composition.png}
    \caption{Both the price crash and the governance attack lead to an under-collateralization of a DeFi lending protocol. In turn, agents will try to exit the protocol by buying other assets (liquidity sweeping). Any agent in a protocol using the now under-collateralized asset as debt, will face the same situation and in turn try to exit via buying other assets (evaporating collateral).}
    \label{fig:composition-cycle}
\end{figure}

\section{Composability and Contagion}
\label{sec:contagion}

% The foregoing has demonstrated how a single DeFi lending protocol may find itself under-collateralized as a result of a sustained downturn in the price of its collateral and reserve assets. 
The possibility of financial contagion in the context of DeFi is of particular importance given the unrestricted composability of protocols~\cite{money-legos}.
In Sections~\ref{sec:stress-test} and~\ref{sec:governance-attack}, we considered an exogenous price drop and a governance attack in each case on a single protocol.
Now we argue why these two design weaknesses can lead to contagion to other protocols that might ultimately lead to a decentralized financial crisis.

Both weaknesses, exogenous price drops and governance attacks, result in the debt asset being under-collateralized.
Assuming rational agents with weak-identities, it is not individually rational for agents to settle their debts, and thus, the under-collateralized asset eventually reaches a value of~0.
Hence, an agent holding such an asset can execute a strategy called \emph{liquidity sweeping} to use his \emph{existing holdings} to buy other assets while the price is not yet~0.
A special sub-case occurs in the governance attack scenario where the attacker can additionally mint an unlimited supply of the debt asset to buy up \textit{all} the available liquidity of other assets. 

Further, any protocol that uses the now under-collateralized asset as a collateral asset to issue another asset, also becomes under-collateralized.
Consider the example of Maker and Compound: Maker uses ETH as a collateral to issue DAI.
Compound allows agents to collateralize DAI to issue a cDAI token.
As DAI becomes under-collateralized, cDAI loses its debt-backing.
We refer to this as \emph{evaporating collateral}.
Holders of any composed assets like cDAI then have to essentially also buy up existing liquidity once they are aware that individually rational agents will not settle their debts.
We illustate this cycle in Fig.~\ref{fig:composition-cycle} and give a total estimate of the financial damage in Fig.~\ref{tab:contagion}.

% The possibility of financial contagion in the context of DeFi is of particular importance given that a defining feature of DeFi is possibility of a financial system comprised of composable protocols~\cite{money-legos}.
% In the following, we consider two channels through which financial contagion could spread in a DeFi economy.
\begin{figure}[tb]
    \centering
    \footnotesize
    \begin{tabularx}{\columnwidth}{Xr}
    \toprule
        \textbf{Weakness} & \textbf{Financial damage (USD)} \\ \midrule
        Under-collateralization (price crash) of MakerDAO & 145m\\
        Under-collateralization (governance attack) of MakerDAO & 211m \\
        Contagious under-collateralization (price crash) of MakerDAO & 180+m \\
        Contagious under-collateralization (governance attack) of MakerDAO & 246+m \\
        \bottomrule
    \end{tabularx}
    \caption{Financial damage for an initial failure of the MakerDAO protocol either through a price crash or a governance attack.}
    \label{tab:contagion}
\end{figure}

% 
\point{Liquidity sweeping}
Contagion occurs when the under-collateralized debt asset is used to ``soak-up'' as much liquidity as possible, before buyers of the debt asset are able to react.
There are two cases:
First, if, as detailed in Section~\ref{sec:stress-test}, the debt asset is under-collateralized due to an exogenous price crash, the agent can trade all their under-collateralized debt (such as DAI) for other assets on DeFi lending protocols which offer liquidity pools such as Compound~\cite{compoundfinance}, Uniswap~\cite{uniswap}, and Aave~\cite{aave}.
This way the agent can dispose of the debt asset if it assumes the debt asset will fall to~0.
% Provided an agent is able to trade all their under-collateralized debt (such as DAI) for other assets on DeFi lending protocols which offer liquidity pools such as Compound~\cite{compoundfinance}, Uniswap~\cite{uniswap} and Aave~\cite{aave}.
Second, if, as detailed in Section~\ref{sec:governance-attack}, an attacker gains the ability to create new tokens without collateral backing, the attacker can use these tokens to buy \emph{all existing liquidity} on available exchanges.
% This contagion mechanism is made worse in the context of Section~\ref{sec:governance-attack}, because with such an attack an attacker would be able to steal \textit{all} of the liquidity on the market, by issuing themselves an unlimited amount of the debt asset.

However, both cases assume that the price of the under-collateralized debt asset is not~0 at least as long to complete the trades.
We support this assumption with the halting of the IOTA cryptocurrency network that occurred on February 13--15,~2020~\cite{iota-status}.
Following a security incident, the IOTA foundation stopped the centralized coordinator such that the IOTA network was not able to process transactions containing value and advised its users to not access their funds in their wallets~\cite{iota-halt}.
On February~15, the attack is still ongoing~\cite{iota-status}.
During the incident, the trading volume on exchanges of IOTA feel from~41m USD to~21m USD.
Notably, the price of IOTA only moved from~0.34 USD to~0.31 USD within~14 hours of the announcement and recovered back to around~0.32 USD after another two hours.
Hence, the inability to transfer the IOTA cryptocurrency and access funds on the IOTA network for an extended period of time, caused only a maximum price drop of~9\%.

To quantify the impact of liquidity sweeping, we took an instantaneous snapshot of major marketplaces offering a DAI pair at approximately noon (GMT+8) on~15 February, as presented in Fig.~\ref{tab:daimarkets}.
In the price crash case, agents could trade the whole of their~\$145m holdings.
However, an agent who had successfully undertaken the governance attack would be able to soak up all of the order book liquidity, since with in effect an unlimited DAI supply they can pay any price to acquire other assets. 
We estimate the total USD value, aggregating across markets and pairs, to be c.~211m USD\footnote{See Appendix~\ref{appendix:contagion} Fig.~\ref{tab:daimarkets}}.

\point{Evaporating collateral}
Liquidity sweeping is not contained to agents that participate in a single lending protocol if the assets of the protocol are used in others as well.
Rather, a vicious cycle occurs where any debt-backed asset issued in another protocols, e.g. where DAI would be used to issue cDAI on Compound, loaned in Aave, and used as a margin trading collateral in dY/dX.
If we consider the DAI example in the price crash case, 145m USD of DAI would be exchanged as well as 35m USD of cDAI and any other protocol that uses DAI as backing collateral.
% One transmission mechanism for financial contagion is where an asset used as collateral in a composable protocol becomes under-collateralized.
% For instance, Compound~\cite{compoundfinance} allows agents to use units of debt, DAI, from the MakerDAO protocol~\cite{makerdao} as collateral, against which they can issue cDAI and earn interest.
% Should DAI become under-collateralized, cDAI would become under-collateralized, resulting in the loss of the debt in the protocol. 

\point{Collateral composition}
As a stylized example, assume that there are $N$ protocols, with different minimum collateralization ratios, that each use $D/N$ as collateral.
In the event of this collateral itself becoming less than~100\% collateralized, we assume that the value of the debt would quickly fall to~0.
We further assume that agents choose a particular protocol for reasons exogenous to the system, and that each agent obtains the maximum leverage they can on a certain protocol by using their issued debt to purchase additional collateral, which in turn is used to issue more debt.
To reflect heterogeneity in collateralization ratios among protocols, we assign each of the $N$ protocols a collateralization ratio based on randomly sampling from a uniform distribution over a specified range.
The maximum possible leverage for a given protocol $\pi$  when an agent allocates $D/N$ units of collateral to it is given by $D/N_{\pi}/\lambda_{\pi}$.
Therefore the maximum systemic loss is given by $\sum_{\pi = 1}^{\Pi}{D/N_{\pi}}/{\lambda_{\pi}}$.

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.8\columnwidth]{images/protocol_defaults.pdf}
    \caption{Financial losses for~30 DeFi protocols, which use the debt asset as collateral. ``O/C'' stands for overcollateralization.}
    \label{fig:protocol_defaults}
\end{figure}

Fig.~\ref{fig:protocol_defaults} demonstrates how for three different maximum overcollateralization parameter ranges, namely~(101--105\%),~(101--150\%), and~(101--300\%), what the maximum system wide losses could be, assuming that the protocol in which the crash occurs has a debt of~400m~USD, and the liquidity parameter is $\rho = 0.01$.
As the minimum overcollateralization ratio falls, the maximum potential losses for the system grow: from right to left, as the minimum overcollateralization requirement falls from~$3\times$ (or~300\%) to~$1.01\times$~(101\%), the maximum possible loss increases.
Given our uniform splitting of debt, what also emerges is that the result is driven by the minimum collateralization ratio.

\point{Crisis}
Agents seek to exit their under-collateralized asset positions by buying other available assets.
Individually rational agents should seek assets that are uncorrelated with the asset they are disposing of.
However, this leads to a spread of the initial DeFi lending protocol failure to any other asset that is available for trading on exchanges that accept the initial lending asset.
Hence, the DeFi crisis can spread across multiple blockchains and also affect centrally-backed assets like USDT~\cite{tether}.


%\point{Interrelation of attacks}

% \begin{itemize}
%     \item Uniswap liquidity pools~\cite{uniswap}, which allow agents to trade ERC20 tokens.
%     \item dYdX permits margin trading for crypto assets, with 4x leverage~\cite{dydx}.
%     \item Aave~\cite{aave} allows agents to lend their assets to, and borrow from, on-chain pools of liquidity.
% \end{itemize

% {\color{blue}
% Add more protocols here. I think affected would be Uniswap liquidity pools; dYdX margin trading pools and borrowing pools, Aave liquidity pools, InstaDApp liquidity pools}


% \point{Uncertainty}
% Make the point that agents may not know which of their assets are fundamentally based on DAI; then draw parallel to the Financial Crisis.

% \point{Impact via market pairs}
% Another transmission mechanism for contagion is through users the market pairs available for the debt asset. [? - Need to reflect]

==> content/mitigation.tex <==
\section{How can the Decentralized Financial risks be mitigated?}\label{sec:risk-mitigation}

Rewind the blockchain.

{\color{blue} If one of the causes of the Fi crisis is transparency, then adding transparency alone does not solve the problems as you can see in DeFi. What if a remedy would be to enforce certain collaterlization and liquidity thresholds [like national banks do FINMA]? In traditional finance, you have rating agencies and financial regulators that check that banks have adequate protections. Would a possible remedy to combine the transparency of blockchain with enforcing similar regulations through the use of smart contracts? I guess we could discuss this.}

\subsection{How the DFC might differ from the GFC}
\label{sec:difference}
\begin{itemize}
    \item Fiscal policy: state has a changed role, and would not be reimbursing actors, good or bad
    \item Monetary policy: what would the role, if any, of a central bank be?
    \item May the central bank be replaced by the biggest token holder? In Maker, the governance mechanism is steered by the token holders..
    \item Key point from \cite{duffie2010failure} that in order to mitigate counterparty risk, some repos are triparty, where the third party is a clearing bank which holds the collateral and is responsible for returning the cash to the creditor. This shields the lender from some of the risk of the borrower's default. Perhaps a trustless protocol would be preferable here, one which could reduce the worst case risk of default by ensuring that some of the liquidation process is automated.
\end{itemize}

[Mention how, similar to the DAO hack, with respect to the governance token it might be possible to reverse the blockchain history --> would this serve to reduce the extent of panic selling (because any lost funds could be restored)? Or does it reduce finality (and generate a risk premium) because agents may not be sure that their trades are final?]
 
See BoE stress testing (DEC 2019). Control timing of capital sell off with open-ended funds.

Should require that DeFi protocols submit to regular stress testing; such stress testing should be publicly verifiable on chain.
Risk should be verifiable on chain.
Credit worthiness should be verifiable on chain.

{\color{blue}
\subsection{Autonomous Regulation}
Regulators in the financial world enforce legislation with the purpose of providing stability in the financial system.
In essence, they ensure that financial institutions have limited financial risk (capital requirements, leverage rates, and liquidity requirements (Basel III etc.)) and reduce operational risks.
[Need a better way to formulate this.]
These requirements are typically implemented through pro-active and reactive controls and audited on a regular basis.
However, with the functionality of smart contracts in DeFi, we could enforce those rules automatically.
For example, one could build a wallet that is compliant with certain financial standards by leveraging the transparency of the underlying blockchain.
That way, one could ensure that the accepted coins comply with the security constraints in~\ref{sec:constraints}.
}


==> notes.tex <==
\section{Other risks [based on talking to others]}

Lack of an insurance body. If MakerDAO collapses, no-one is protecting users' funds (there is no lender of last resort).

Dominik: most interesting would be to verify the risks. The first problem is that we don't know what the risks are. Then even once we know what the risks are, there are incentive issues surrounding whether the risks are being accurately reported etc. 

[MKR tokens, absolute failure of underlying coin - a buffer. Try to buy back governance tokens at a higher price before they get too expensive. DAO hack June July 2017.
Right now assumption is underlying coin fails. what if a protocol fails on top of ethereum so badly that you hard fork your coin? 20\% locked in the DAO; Eth/eth classic. From a risk modelling point of view, if a protocol fails on top, can affect underlying coin. Feedback effects defi layer and base layer. Two way feedback between defi. ]

[zerocoin - inflation bug, you could print money
zcash - issues
bitcoin - https://en.bitcoin.it/wiki/Common_Vulnerabilities_and_Exposures
list incidents where this has happened - see whether there is a correlation between the incident and the price of the underlying asset.
see pump and dump paper
collect data on case studies
predicting decentralized financial crisis
follow pump and dump structure
what are the price implications if a defi protocol breaks down (would need to make strong assumptions)]

{factor in the dominance of DAI on DeFi pulse}
{show bound beyond which a defi protocol could collapse - if insufficient liquidity on orderbook to sell off a cryptocurrency that underlies a protocol - can characterize with parameters - if larger than share $\rho$ over time period $x$ then defi architecture doomed to failure. Remedy - capital limits to within safe params. Need an assessment of failure risk.}

\subsection{The Evaporation of Confidence in the Market}

-Intrinsic to the value of an asset is the belief that the asset will continue to be valuable in the future, that is, others will continue to value the asset in the future.
-One difference between fiat currencies and cryptocurrencies as collateral is that cryptocurrencies can suddenly lose value for fundamental reasons. For example, a fatal flaw could be discovered in the ETH protocol, or the Bitcoin protocol, etc. 
- While the probability of such a flaw is small, it is not 0, and moreover prima facie it seems to be much higher than the probability of the US Dollar using value for some fundamental reason. 
- Indeed, plausibly the dollar cannot lose value for some fundamental reason. 
- Moreover in the scenario where ETH collapses, it is easy to switch to another cryptocurrency to make transactions, or another currency altogether. To some extent, cryptocurrencies are substitutes for each other. 
- In contrast and for this reason, it is difficult for the US dollar to collapse, because e.g. in the USA it is difficult to see how another means of exchange would be used; people still need to use US dollars. 
\textbf{Unlike fiat, crypto seems to be much more vulnerable to binary failures, where suddenly it is discovered that the whole currency is fatally flawed.}


% List of big crypto bugs (not exhaustive but the worst ones)
% \begin{itemize}
%     \item Zerocoin and the inflation bug [https://zcoin.io/zcoins-zerocoin-bug-explained-in-detail/]
%     \item the DAO hack
%     \item the parity hack
% \end{itemize}

==> old.tex <==
\begin{itemize}
    \item funds borrowed on platform x (e.g. Maker DAO DAI) used as collateral in another loan (e.g. on Compound). If CDP becomes undercollateralized, then secondary market loan becomes invalid (make a figure. cDAI acceptee needs to check that the cDAI is still a valid CDP. If you accept something on an exchange you need to follow the history of the coin. But this may not be possible on current exchanges. Do exchanges take care of this? Do they do this? Especially if you have a DEX, what is the difference?Boils down to Bitcoin - need to check whether outputs are spent or not. A blockchain in a blockchain? cDAI needs to see if the DAI still exists)
    \item {\color{blue} [Explanatory/non-final text!] the value of 1 DAI remains at 1 USD/DAI, provided the system is sufficiently collateralized as a whole. A DAI is a completely fungible ERC-20 token. Indeed, to repay a DAI debt, users can buy DAI on the open market and use it to repay their debt denominated in DAI. As such, there is no need to be concerned about the collateral backing one specific unit of DAI, because if the CDP that originally generated the DAI becomes under collateralized and enters liquidation, the generated DAI is untouched and instead 113\% of the DAI debt value in PETH is seized and auctioned off for DAI on the Maker dashboard. The DAI received from the sale is then burned, wiping out the liability of the DAI debt. So 1 DAI has the value of approximately 1 USD provided the \emph{system as a whole} is sufficiently collateralized.
    \item if the price of ETH drops sufficiently fast or is gapped (e.g., what if multiple eth exchanges are taken down at the same time), perhaps the system as a whole could become undercollateralized. This would then undermine the tertiary markets built on top of DAI, e.g. the value of cDAI would change. So cDAI inherits this risk from DAI. Perhaps this makes a case for decentralized exchanges?}
    \item over-leverage is particularly the case if borrowed funds are used to buy more of the underlying collateral (e.g. Maker DAO you can get up to 4.5x leverage)
    \item insufficiently incentivized `liquidators' to buy undercollateralized positions, due to loss of confidence in a particular asset
    \item misunderstood dynamics of multi-collateralized debt positions (e.g. potential with Maker DAO MCD), resulting in mis-estimation of the minimum required collateralization levels
    \item Getting the collateralization levels wrong for a specific collateral type (too low, resulting in loss, too high resulting in inefficiency)
    \item {\color{blue} in MakerDAO, there is the additional risk of holding PETH as opposed to ETH as collateral, since in the event of a price crash the user may not actually be able to redeem their ETH 1:1}
    \item ~\cite{stiglitz2010interpreting} the risk of correlated behaviours, see p. 5
    \item Related to Repos, what about the risk that the Dai just isn't repaid? There is no expiry term on a Dai repurchase agreement - does this lay the foundation for an intrinsic bubble? 
\end{itemize}


\paragraph{Default of a base institution}.
Consider the failure of Dai, when this asset underlies a secondary market such as a secondary lending market on compound.
Dai is an asset backed decentralized stablecoin provided by the Maker Foundation~\cite{makerdao}.
A borrower with ETH holdings can interact with the MakerDAO platform and issue themselves with DAI, posting 150\% of the amount that they wish to borrow in DAI (where DAI maintains a soft peg with the US Dollar).
For instance, to borrow \$100 of DAI, the user must post at least 150 USD of ETH. 
Such borrowed DAI may be used to gain access to short-term funding, or for leverage and increased exposure to ETH if the DAI is used to repurchase ETH. 



\subsection{Other risks}
\label{sec:regulatoryrisk}

\paragraph{Blockchain risk}
{\color{red}Goal: quantify what's the worst possible thing that can happen in a DFC (based on a technical risk)}

\paragraph{Layer-zero}

\begin{itemize}
    \item Hardware vulnerabilities (Intel SGX vulnerabilties){\color{red}Bitcoin/Ethereum should not be affected by that}
    \item Eclipse attack
    \item DNS Hijacks
    \item BGP Hijacks
    \item DDoS attack
\end{itemize}

\paragraph{Layer-one attacks}

\begin{itemize}
    \item 51\% attack
    \item Selfish mining attack
    \item Double-spending
    \item Consensus Delay
    \item Timejacking
    \item Finney attacks
    \item Smart-contract vulnerabilities (reentrancy, overflow, replay, short address, balance)
\end{itemize}

\paragraph{Layer-two attacks}

\begin{itemize}
    \item Wormhole attack
    \item Theft of funds from unwatched channel
    \item Malicious operator
\end{itemize}
\paragraph{Regulatory risk}
\begin{itemize}
    \item Blockchain ban?
    \item Can a country ban a smart contract, but not the blockchain itself?
    \item KYC could be enforced on any blockchain node which ``helps'' to enact transactions.
\end{itemize}

\paragraph{Governance risk}
Governance risks particularly pertinent to MakerDAO where Maker Token holders could opt for global settlement. 

\paragraph{Oracle attacks}

\begin{itemize}
    \item Oracle attack - e.g. Price Feeds into a debt system are hijacked, corrupting the reported market price
    \item Gaming oracle update frequency ('The missing money attack'). If an Oracle updates the system reference price in expectation every x seconds, in the interval debt positions could be deliberately undercollateralized (high frequency algorithmic trading) such that the capital is used elsewhere. Oracle updates provide checkpoints: the more frequent they are the more secure the system
\end{itemize}

\paragraph{Liquidity risk}

\begin{itemize}
    \item Markets becoming illiquid, assets taking a large haircut on final price
    \item Possibility of multiple exchanges going down at the same time
\end{itemize}

\paragraph{Custodian risk}

\begin{itemize}
    \item Exchange hacks resulting in loss of funds
\end{itemize}

\paragraph{On-Chain Exchanges}
\begin{itemize}
    \item Front-running and other market manipulation
\end{itemize}


% \subsubsection{Seven Stages of a Long-Term Debt Cycle}\label{sec:debt-cycle-components}
% Analyzing economic data is typically easiest in hindsight. Related work has thoroughly analyzed cycles, in particular $48$ individual long-term debt cycles~\cite{dalio2018principles}. Dalio characterizes the seven stages of an archetypal long-term debt cycle as follows:

% %In (i) the early part of the cycle
% \begin{description}
% \item[Early Part of the Cycle]
% \item[Bubble]
% \item[Top]
% \item[Depression]
% \item[Deleveraging]
% \item[Normalization]
% \end{description}

%\subsection{Identifying Bubbles}
%\begin{description}
%\item[Have new participants entered the market?]
%\item[Is there a broad bullish sentiment?]
%\item[Does tightening (by policy makers) risk popping the bubble?]
%\item[Are prices high relative to traditional measures?]
%\item[Are prices discounting future rapid price appreciation?]
%\item[Are purchases being financed by high leverages?]
%\item[Are buyers/companies making forward purchases?]
%\end{description}

%\subsection{Identifying Bubbles}
%\begin{description}
%\item[Have new participants entered the market?]
%\item[Is there a broad bullish sentiment?]
%\item[Does tightening (by policy makers) risk popping the bubble?]
%\item[Are prices high relative to traditional measures?]
%\item[Are prices discounting future rapid price appreciation?]
%\item[Are purchases being financed by high leverages?]
%\item[Are buyers/companies making forward purchases?]
%\end{description} typically smaller than the long-term debt cycle. Over-posing productivity growth, with short and long-term debt cycles yields the results of Figure [].


\subsection{Debt cycles in DeFi}

% {\color{red}
% which phases are the cycles composed of?
% what current metrics are being taken to identify in which cycle the state of the cryptoeconomy?
% which ones do we propose?
% }

\begin{itemize}
    \item In the long run, we expect the debt cycles as described in \ref{sec:debt-cycle-components} to occur in a financial system based on DeFi
    \item Even now, we see early evidence of such cycles in cryptocurrencies, although these are not at present plausibly driven by debt, instead by speculative interest
    \item It is clear, therefore, that a DeFi architecture needs to be able to withstand such cycles
    \item In particular, a DeFi system needs to be able to weather the bursting of bubbles, whatever the source (debt or speculative interest, possibly both)
\end{itemize}

This paper is the first to systematically characterize the risks that are inherent to DeFi.
At an abstract level, reflecting core principles of the operation of DeFi protocols, we characterize the constraints on a DeFi protocol required to ensure its financial security.
With a specific focus on DeFi lending protocols, we then leverage Monte Carlo simulation to examine how a severe tail event could cause a DeFi lending protocol to become undercollateralized, triggering its own collapse. 
Further, we simulate the effects of financial contagion in the presence of composable DeFi protocols and examine how the collpase of one DeFi protocol could lead to a complete DeFi meltdown. 
At a concrete level, we examine the security of MakerDAO, currently the largest DeFi lending platform, and show how two attack vectors on the MakerDAO governance mechanism, the Crowdsourcing Attack and the Liquidity Pool Attack, could feasibly allow an adversary to steal the funds in escrow.
Such attacks could themselves trigger a Decentralized Financial Crisis. 
